MiniVLM: A Smaller and Faster Vision-Language Model

Recent vision-language (VL) studies have shown remarkable progress by learning generic representations from massive image-text pairs with transformer models and then fine-tuning on downstream VL tasks. While existing research has been focused on achieving high accuracy with large pre-trained models, building a lightweight model is of great value in practice but is less explored. In this paper, we propose a smaller and faster VL model, MiniVLM, which can be finetuned with good performance on various downstream tasks like its larger counterpart. MiniVLM consists of two modules, a vision feature extractor and a transformer-based vision-language fusion module. We design a Two-stage Efficient feature Extractor (TEE), inspired by the one-stage EfficientDet network, to significantly reduce the time cost of visual feature extraction by $95\%$, compared to a baseline model. We adopt the MiniLM structure to reduce the computation cost of the transformer module after comparing different compact BERT models. In addition, we improve the MiniVLM pre-training by adding $7M$ Open Images data, which are pseudo-labeled by a state-of-the-art captioning model. We also pre-train with high-quality image tags obtained from a strong tagging model to enhance cross-modality alignment. The large models are used offline without adding any overhead in fine-tuning and inference. With the above design choices, our MiniVLM reduces the model size by $73\%$ and the inference time cost by $94\%$ while being able to retain $94-97\%$ of the accuracy on multiple VL tasks. We hope that MiniVLM helps ease the use of the state-of-the-art VL research for on-the-edge applications.

==> tables.tex <==


% \begin{table*}[h!]
% \begin{center}
% \caption{VQA 2.0 evaluation results (single model) on validation and test-dev sets}
% \scriptsize
% \label{tab:vqa}
% \begin{tabular}{l@{\hspace{3mm}}|c@{\hspace{3mm}}c@{\hspace{3mm}}c@{\hspace{3mm}}|c@{\hspace{3mm}}c}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{3}{c|}{computation cost} & \multicolumn{2}{c}{accuracy}\\ 
% & \#Params & \#FLOPs & Time & vqa-eval & test-dev\\
% \midrule
% BUTD~\cite{00010BT0GZ18} & & & & $63.2$ & - \\
% ResNet-50 Grid~\cite{jiang2020defense}  & & & & $64.37$ & - \\
% ResNeXt-101 Grid + Pythia~\cite{jiang2020defense}  & & & & - & $67.76$ \\
% ResNeXt-101 Grid + MCAN~\cite{jiang2020defense}  & & & & - & $72.59$ \\
% Oscar$_{\text{B}}$~\cite{Li0LZHZWH0WCG20} & & &  & - & $73.16$\\
% \midrule
% Ours  & & &  & $66.3$ &  \\
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table*}

% \begin{table*}[h!]
% \begin{center}
% \caption{Inference time breakdown. Our model architecture can achieve competitive results on image captioning (VQA?) while being $???\times$ faster, by reducing tremendous time cost in ....}
% \scriptsize
% \label{tab:time_breakdown}
% \begin{tabular}{l@{\hspace{3mm}}|c@{\hspace{3mm}}c@{\hspace{3mm}}|c@{\hspace{3mm}}c@{\hspace{3mm}}|c@{\hspace{3mm}}c@{\hspace{3mm}}c}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{2}{c|}{settings}  & \multicolumn{2}{c|}{performance} & \multicolumn{3}{c}{inference time breakdown}\\ 
% & input size & \#features & mAP & CIDEr & OD & caption & total\\
% \midrule
% BUTD~\cite{00010BT0GZ18} & & & & & & &  \\
% Grid~\cite{jiang2020defense} & & & & & & &  \\
% Oscar$_{\text{B}}$~\cite{Li0LZHZWH0WCG20}& & & & & & & \\
% \midrule
% Ours & & & & & & & \\
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table*}

% \begin{table*}[t!]
% \begin{center}
% \caption{
% Comparison of models with and without vision-language pre-training on downstream tasks. With the compact model structure, our pre-training is still able to benefit from both larger vision datasets and larger VL datasets.}
% \scriptsize
% \label{tab:vlp}
% \begin{tabular}{cc|ccc|ccc|cccc|cc|c|c}
% \toprule
% \multicolumn{2}{c|}{Pretraining datasets} & \multicolumn{3}{c|}{Image Retrieval} & \multicolumn{3}{c|}{Text Retrieval} & \multicolumn{4}{c|}{Image Captioning} & \multicolumn{2}{c|}{NoCaps} & VQA & NLVR2 \\ 
% vision data & VL data & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & B@4 & M & C & S & C & S & test-std & test-P\\ \midrule
% 
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table*}
